Privacy Accounting and Quality Control in the Sage Differentially Private ML Platform

Companies increasingly expose machine learning (ML) models trained over sensitive user data to untrusted domains, such as end-user devices and wide-access model stores. We present Sage, a differentially private (DP) ML platform that bounds the cumulative leakage of training data through models. Sage builds upon the rich literature on DP ML algorithms and contributes pragmatic solutions to two of the most pressing systems challenges of global DP: running out of privacy budget and the privacy-utility tradeoff. To address the former, we develop block composition, a new privacy loss accounting method that leverages the growing database regime of ML workloads to keep training models endlessly on a sensitive data stream while enforcing a global DP guarantee for the stream. To address the latter, we develop privacy-adaptive training, a process that trains a model on growing amounts of data and/or with increasing privacy parameters until, with high probability, the model meets developer-configured quality criteria. They illustrate how a systems focus on characteristics of ML workloads enables pragmatic solutions that are not apparent when one focuses on individual algorithms, as most DP ML literature does.

==> sections/limitations.tex <==


\heading{Event-Level Privacy.}
Motivated by our desire to overcome difficult challenges of global DP -- including running out of privacy budget, which we believe is a real roadblock to DP adoption -- we focused this paper and evaluation on event-level DP, for which we believe these challenges can indeed be addressed practically.
However, we acknowledge that this semantic has significant limitations when groups of correlated observations can reveal sensitive information.
The best known example of such correlation happens when a user contributes multiple observations, but other examples include repeated measurements of a phenomenon over time, or users and their friends on a social network.
In such cases observations are all correlated and can reveal sensitive information (e.g. a user's demographic attributes) despite event-level DP.
However, even in the face of correlated data DP holds for each individual
observation: other correlated observations constitute side information, to which
DP is known to be resilient.
Event-level DP also provides some protection to groups of observations through group
privacy~\cite{dwork2014algorithmic}, but these guarantees degrade exponentially with group size.

\iffalse
Using semantics such as user-level DP, which enforces the DP guarantee
(Def. \ref{def:dp}) over all observations of a user, would provide stronger
guarantees.
\S\ref{sec:block-composition} includes a discussion of how user-level privacy can be supported with our theory and system design.  The challenge is that the central requirement for not running out of privacy budget in DP -- that the database grows fast enough in terms of new blocks -- is unlikely to be met with a user-level semantic.
\fi

\heading{DP Budget Management.}
A key practical question when training DP models is to choose the DP
parameters ($\epsilon$, $\delta$) and number of data points to allocate to each
model, to conserve privacy budget while reaching quality targets.
\sysname proposes and evaluates a heuristic to perform this allocation
(\S\ref{sec:sage-iterative-training},
\S\ref{sec:evaluation:end-to-end-experiment}) but identifying principled approaches to perform these allocations remains an open problem.
We suspect that resource allocation literature from systems will be relevant.

Furthermore, \sysname impacts traditional resources.
Some DP training techniques can be slower than their non DP equivalent. For
instance, DP SGD involves sampling batches without replacement which is slower
than the typical shuffle and loop approach used in deep learning.
Computing per-example gradients for DP SGD is also computationally intensive.
More specific to \sysname's approach, \iterativetraining requires training each model multiple times.
The management and allocation of compute resources in the context of \sysname is a
promising direction for systems support of DP ML.

\iffalse
\heading{DP Programmability.}
Another important direction of future work is to identify solid programming models for DP ML pipelines.  This paper has completely ignored the difficulty of composing such pipelines, assuming that sufficient literature exists for (informed) developers to safely put together DP training pipelines.
Research into new programming and testing support is needed to avoid programming errors that spoil the DP guarantee.
\fi


==> sections/system-description/dp-validation-tests.tex <==
\begin{lstlisting}[float,floatplacement=tbp,
label={list:dp_validator},
language=Python,
caption={\bf Example DPModelValidator used in \L\ref{list:dp_pipeline}.}]
class DPLossValidator(DPModelValidator):
  def bernstein_ub(self, loss, n, eta, B):
    return loss + sqrt(2*B*loss*log(1/eta)/n) +
           4*log(1/eta)/n

  def hoeffding_lb(self, loss, n, eta, B):
    return loss - B*sqrt(log(1/eta)/n)

  def _validate(train_labels, eval_labels,
    dp_eval_predictions, np_train_predictions,
    quality_target, privacy_budget, confidence,
    loss_fn, B):
    # We will do 2 DP test of each dataset, and
    # Two statistical tests for ACCEPT/REJECT.
    eps = privacy_budget / 2
    eta = confidence / 2
    # ACCEPT test
    dp_eval_loss = clip_by_value(loss_fn(eval_labels,
      dp_eval_predictions), 0, B) + lapalce(B/eps)
    corrected_dp_eval_loss = dp_eval_loss +
                             B*log(3/eta)/eps
    n_test = dp_test_predictions.size()
    n_tot = n_test + lapalce(1/eps)
    corrected_n_tot = n_tot + log(3/eta)/eps
    if self.bernstein_ub(
        corrected_dp_eval_loss / corrected_n_tot,
        n_tot, eta / 3, B
        ) <= quality_target:
      return ACCEPT
    # REJECT test
    n_train = dp_train_predictions.size()
    n_tot = n_train + lapalce(1/eps)
    n_tot_min = n_tot - log(6/eta) / eps
    n_tot_max = n_tot + log(6/eta) / eps
    dp_train_loss = clip_by_value(loss_fn(train_labels,
      dp_train_predictions), 0, B)
    corrected_dp_train_loss = dp_train_loss +
      lapalce(B/eps) - B*log(3/eta)/eps
    if self.hoeffding_lb(
        corrected_dp_train_loss / n_tot_max,
        n_tot_min, eta / 3, B
        ) > quality_target:
      return REJECT
    # Neither ACCEPTed nor REJECTed
    return RETRY
\end{lstlisting}

\heading{Model Validation Semantics:}
Model validation in \sysname provides three key semantics to the system's user.
First, trained models need to be evaluated, and accepted only when their performance
on new data will be good enough.
To do this, \sysname provides an acceptance test.
This test takes a performance metric (e.g. accuracy), performance goal, and candidate model.
\sysname then runs a differently private statistical test on a test set.
At a high level, if the model passes this test, it ensures that with high probability, the model's
performance on new data will be the performance goal of higher.
Because this is a statistical test, there is a configurable probability of failure. This probability
of failure is over the randomness in the sampled data and the DP noise. The smaller the
probability of failure, the more data is needed in the testing set to clear the test.

Second, it is possible that performance goals are too high, and no model in the considered model class
could reach this performance.
\sysname provides a rejection test to stop increasing the privacy budget and data used when this is the
case. Intuitively, the model trained on the training set provides an error that is smaller than the error
on general data, because it was able to (over)fit the data as closely as possible. \sysname then runs a
differently private statistical test on the training test to computes bounds on how well any model in the
same model class could hope to do on new data. If this test shows with high probability that the performance
objective can never be reached, the model is rejected and the iterative training procedure stops.


Third, these validation procedures need to be differentially private. The acceptance test
use DP models, and evaluate their performance on a testing set. The procedure needs to be
DP with regards to the testing set. The rejection test uses only data from the training set,
and thus needs to be DP with regards to the training data. It is important that \sysname accounts
for the privacy budget use on the correct part of the data. Moreover, the DP noise will impact
the statistical tests used for validation: we thus adapt these tests to provide the previously
described semantics despite the DP noise.

Finally, we note that the performance goal may be an absolute value, but also an
existing model to compare to.  In this case, the performance on each data point
is measured as the difference in the score of the condidate model and the score
of the comparison model.


\heading{Example Model Validators:}
\sysname provides built-in model validators for three different objectives: accuracy goals, loss value goals, and sum based summary statistics (e.g. mean, variance).
At a high level, these validators all follow the same logic. For validation, first compute a DP version of the test quantity (e.g. the accuracy), usually on a testing set. Second, compute the worst case impact of DP noise on that quantity for a given confidence probability. For instance, if we added Laplace noise with parameter $\frac{1}{\epsilon}$ to the accuracy on $n$ data points, we know that with probability $(1-\eta)$ the accuracy is inflated by less than $\frac{\ln(1/\eta)}{\epsilon}$, because a draw from this Laplace distribution has just a $\eta$ probabiulity to be larger that this value.
Third, use existing statistical concentration inequalities to bound with high probability the accuracy of the model on the entire distribution based on its (corrected for worst case DP impact) results on the testing set.
Users of \sysname can thus follow the same logic for different problem types or metrics to create new validators.
Each validator relies on specific statistical bounds, and could be done differently, which may be better depending on the specifics of the problem.

We next detail \sysname's built-in validators, that provide useful defaults and show the reasoning to create new validators.
To formalize \sysname's validators, we use the following notation: we use $f$ for a model form a familly of models $\mathcal{F}$. An objective to minimize, often called risk or loss, is noted as $l(f, x, y)$ for a given datapoint (here $f$ is the model, $x$ the data point, $y$ the true answer), and we note $\mathcal{L}_{\D}(f) = \mathbb{E}_{(x,y)\sim \D x \Y}(l(f, x, y))$ the expected loss of $f$ on the data distribution, $\mathcal{\hat L}_{tr}(f) = \frac{1}{n_{tr}} \sum{i=1}^{n_{tr}} l(f, x_i, y_i)$ and $\mathcal{\hat L}_{te}(f)$ the emprirical loss on the training and testing sets respectively. Similarly, we note $f^*$ the best possible model on the data distribution ($f^*$ minimizes $\mathcal{L}_{\D}(f)$), and $\hat f$ the best model on the training set ($\hat f$ minimizes $\mathcal{\hat L}_{tr}(f)$).

The {\em Accuracy Validator} applies to classification problems, where a model
$f: \X \rightarrow \Y$ maps data points in space $\X$ to one of multiple
possible categories in $\Y$.
The objective is expressed in terms of accuracy, the proportion of correct
predictions:  $l(f, x, y) = \mathbb{1}\{f(x) = y\}$ and $\mathcal{\hat L}(f) =
\frac{1}{n} \sum_n \mathbb{1}\{f(x) = y\}$, where $y$ is the true label, and
$\mathbb{1}\{\text{predicate}\}$ is the indicator function with value $1$ if the
predicate is true, and $0$ otherwise.
  We note $\underline{\text{Bin}}(n_{heads}, n_{tot}, \eta)$ the lower bound on the probaility parameter $p$ of a binomial distribution such that $n_{heads}$ happen can happen with probability at least $\eta$ out of $n_{tot}$ independent draws. Simalarly $\overline{\text{Bin}}(n_{heads}, n_{tot}, \eta)$ is the upper bound. Both can be conservatively approximated using a Clopper-Pearson interval.

\begin{proposition}[Accuracy Acceptance Test]\label{prop:acc-test}
  Given an accuracy objective $\tau_{acc}$, a testing set of $n_{te}$ i.i.d. samples, a model $f$ is accepted if:
  \begin{align*}
    \underline{\text{Bin}}\Big(n_{true} & - \frac{\ln(3/\eta)}{\epsilon_1}, n_{tot} + \frac{\ln(3/\eta)}{\epsilon_2}, \frac{\eta}{3}\Big) \geq \tau_{acc} ,\\
    \text{Where:} \ n_{true} & = \sum_{n_{te}} \mathbb{1}\{f(x) = y\} + Laplace(\frac{1}{\epsilon_1}) , \\
    n_{tot} & =  {n_{te}} + Laplace(\frac{1}{\epsilon_2}) .
  \end{align*}
  The test is $(\epsilon_1 + \epsilon_2, 0)$-DP w.r.t. the testing set.
  If $f$ is accepted, then with probability at least $(1-\eta)$, the accuracy over the data distribution is at least $\tau_{acc}$: $\mathcal{L}_{\D}(f) \geq \tau_{acc}$.
\end{proposition}
\begin{proof}
  The only data interaction are to compute $n_{true}$ and $n_{tot}$, those are two queries with sensitivity $1$, and performing both with the Laplace noise added is $(\epsilon_1 + \epsilon_2, 0)$-DP.
  With probability at least $(1-\frac{\eta}{3})$ $n_{true} \geq \mathbb{1}\{f(x) = y\}$, which means that $n_{true} - \frac{\ln(3/\eta)}{\epsilon_1}$ is a lower bound on number of true predictions with that probability.
  Similarly, $n_{tot} + \frac{\ln(3/\eta)}{\epsilon_2}$ is an upper bound on the total number of observations.
  Because everything else being equal $\underline{\text{Bin}}()$ is increasing in $n_{true}$ and decreasing in $n_{tot}$, the left hand side of the first line computes a lower bound on the accuracy with proability $\frac{\eta}{3}$.
  Applying a union bound over those three tests, the test passes if with probability at least $(1-\eta)$ the accuracy is higher than $\tau_{acc}$.
\end{proof}

\begin{proposition}[Accuracy Rejection Test]
  With $\hat f$ the best model on the training set of $n_{te}$ i.i.d. samples, a model $f$ is rejected if:
  \begin{align*}
    \overline{\text{Bin}}\Big(n_{true} & + \frac{\ln(3/\eta)}{\epsilon_1}, n_{tot} - \frac{\ln(3/\eta)}{\epsilon_2}, \frac{\eta}{3}\Big) < \tau_{acc} ,\\
    \text{Where:} \ n_{true} & = \sum_{n_{tr}} \mathbb{1}\{\hat f(x) = y\} + Laplace(\frac{1}{\epsilon_1}) , \\
    n_{tot} & =  {n_{tr}} + Laplace(\frac{1}{\epsilon_2}) .
  \end{align*}
  Note that the test is performed on $\hat f$ not the candidate model, because it makes a statement on the whole model class.
  The test is $(\epsilon_1 + \epsilon_2, 0)$-DP w.r.t. the testing set.
  If $f$ is rejected, then with probability at least $(1-\eta)$, the best possible accuracy over the data distribution is bellow $\tau_{acc}$: $\mathcal{L}_{\D}(f^*) < \tau_{acc}$.
\end{proposition}
\begin{proof}
  To show that the procedure is $(\epsilon_1 + \epsilon_2, 0)$-DP, we need to show that computing $\hat f$ and then $n_{true}$, has sensitivity $1$. $\hat f = \arg\max_f \sum_{n_{tr}} \mathbb{1}\{\hat f(x) = y\}$. If we add a apoint to the training set, the $\hat f$ of the previous dataset has the same accuracy on the points in common, and at wose is wrong on the new point. So the $\arg\max$ model on this new dataset can at worse make one more error, or it would not be the best (i.e. the $\arg\max$).  The argument when removing a point is symmetric.
  Hence the sensitivty of finding $\hat f$ and evaluating it on the training set has sensitivity $1$.
  \\
  Because $\hat f$ is the function with the best accuracy on the training set, it has better accuracy on that set than $f^*$, the best model on the whole distribution, so $n_{true}^{\hat f} \geq n_{true}^{\hat f^*}$.
  Then by the same reasoning as in Proposition \ref{prop:acc-test}, this computes an upper bound on the accuracy of $f^*$ on the data distribution. If the best possible model $f^*$ cannot reach the objective $\tau_{acc}$, we reject the model.
\end{proof}
Note that in practice, it is not possible to compute $\hat f$ in many cases (e.g. the optimization problem is non convex, or the objective is computationally hard to optimize, as is the case with accuracy). In practice, we use the result of the non-DP optimization to approximate $\hat f$. This is a good heuristic that works in practice, but can lead to wrong rejections is $\hat f$ is far from the optimal. The procedure is still differentially private as long as adding or removing a data point doesn't yield a worse performance on the other points.

Another typical way to train and evaluate ML models is to use a loss function that penalizes bad predictions (so a lower loss is better).  The {\em Loss Validator} applies to this use case, which covers regression (e.g. mean squared error), classification (e.g. log loss), and many unsupervised settings (e.g. log likelyhood of a Bayesian generative model).
The loss validator follows the exact same logic as the accuracy validator, with two small changes. First, the upper and lower bounds are reversed as losses are minimized while accuracy is maximized. Second, predictions do not follow a binomial distribution, and we have to use different startistical bounds. We typically use Hoeffding's inequality \cite{hoeffding1963probability}, Bernstein's inequality \cite{Shalev-Shwartz:2014:UML:2621980} when we expect the loss to be very small, or empirical Bernstein bounds \cite{2009arXiv0907.3740M} when we expect the variance to be small.
Other bounds may give tighter results in specific cases.

\begin{proposition}[Loss Acceptance Test]
  Given a loss objective $\tau_{loss}$, a testing set of $n_{te}$ i.i.d. samples, a loss function $l$ bounded by $B$, a model $f$ is accepted if:
  \begin{align*}
    \mathcal{L}_{te}(f)  & + \sqrt{\frac{2 B \mathcal{L}_{te}(f) \log(3/\eta)}{n_{tot}}} + \frac{4 \log(3/\eta)}{n_{tot}} \leq \tau_{loss} \\
    \text{Where:} \ n_{tot} & =  {n_{te}} + Laplace(\frac{1}{\epsilon_2}) - \frac{\log(3/\eta)}{\epsilon_2}, \\
    \mathcal{L}_{te}(f) & = \frac{1}{n_{tot}} \Big( \sum_{n_{te}} l(f, x, y) + Laplace(\frac{B}{\epsilon_1}) + \frac{B\log(3/\eta)}{\epsilon_1} \Big) .
  \end{align*}
  The test is $(\epsilon_1 + \epsilon_2, 0)$-DP w.r.t. the testing set.
  If $f$ is accepted, then with probability at least $(1-\eta)$, the expected loss over the data distribution is at most $\tau_{loss}$: $\mathcal{L}_{\D}(f) \leq \tau_{loss}$.
\end{proposition}

\begin{proposition}[Loss Rejection Test]
  With $\hat f$ the best model on the training set of $n_{tr}$ i.i.d. samples, a model $f$ is rejected if:
  \begin{align*}
    \mathcal{L}_{tr}(\hat f)  & - B \sqrt{\frac{\log(3/\eta)}{n^{min}_{tot}}} > \tau_{loss} , \\
    \text{Where:} \ n^{min}_{tot} & =  {n_{tr}} + Laplace(\frac{1}{\epsilon_2}) - \frac{\log(6/\eta)}{\epsilon_2}, \\
    n^{max}_{tot} & =  {n_{tr}} + Laplace(\frac{1}{\epsilon_2}) + \frac{\log(6/\eta)}{\epsilon_2}, \\
    \mathcal{L}_{tr}(\hat f) = \frac{1}{n^{max}_{tot}} & \Big( \sum_{n_{te}} l(f, x, y) + Laplace(\frac{B}{\epsilon_1}) + \frac{B\log(3/\eta)}{\epsilon_1} \Big) .
  \end{align*}
  The test is $(\epsilon_1 + \epsilon_2, 0)$-DP w.r.t. the testing set.
  If $f$ is rejected, then with probability at least $(1-\eta)$, the best possible expected loss over the data distribution is above $\tau_{loss}$: $\mathcal{L}_{\D}(f^*) > \tau_{loss}$.
\end{proposition}

Finally, \sysname provides a {\em Sum Based Statistics Validator}. This validator is slightly different. First, the goal is to approximate a given sum based statistics (e.g. mean, variance) within a satisfactory error $\tau_{err}$: this error can be computed directly on the training set, so there is no need to a test set. Second, because of the law of large numbers, we can always reach the target precision, so there is no rejection test.
We next show the tests using empirical Bernstein bounds \cite{2009arXiv0907.3740M}.

\begin{proposition}[Sum Based Statistics Acceptance Test]
  Given an error objective $\tau_{loss}$ and a testing set of $n_{te}$ i.i.d. samples, the sum of feature values with bounded range $x \in [a, b]$ is accepted if:
  \begin{align*}
    & \sqrt{\frac{2 \mathbb{V}_{tr}(x) \log(6/\eta)}{n_{tot}}} + \frac{7 \log(6/\eta)}{3 (n_{tot} - 1)} \leq \tau_{err} \\
    \text{Where:} \ n_{tot} = & {n_{te}} + Laplace(\frac{1}{\epsilon_2}) - \frac{\log(3/\eta)}{\epsilon_2}, \\
    \mathbb{V}_{tr}(f) = & \frac{1}{n_{tot} (n_{tot} - 1)} \sum_{n_{te}} (x - \sum_{n_{te}} x) ^ 2 \\
    & + Laplace(\frac{b-a}{\epsilon_1}) + \frac{\log(3/\eta)(b-a)}{\epsilon_1} .
  \end{align*}
  The test is $(\epsilon_1 + \epsilon_2, 0)$-DP w.r.t. the testing set.
  If the summary statistic is accepted, then with probability at least $(1-\eta)$, the expected additive error on the value over the distribution is bellow $\tau_{err}$.
\end{proposition}




==> sections/system-description/slaed-model-validation.tex <==


\sysname's model validation accounts for DP randomness to provide a statistical guarantee of correct positive assessment.
We call the process {\em SLAed model validation} because the guarantee resembles a quality service level agreement (SLA).
\F\ref{fig:sage-architecture} shows the three possible outcomes of SLAed model validation: {\ACCEPT}, {\REJECT}, and {\RETRY}.
If SLAed model validation returns {\ACCEPT}, then with high probability (e.g. 95\%) the model reaches its configured quality targets when predicting on new data from the same distribution.
For certain metrics and under certain assumptions, it is also possible to give statistical guarantees of correct negative assessment.
In such cases, if SLAed validation returns {\REJECT}, then with high probability (e.g., 95\%) this type of model {\em will never} reach the configured target, no matter how much data it is trained/validated on.
Finally, if SLAed validation returns {\RETRY}, it signals that it needs more data for an assessment.



\begin{lstlisting}[float,floatplacement=tbp,
label={list:dp_validator},
language=Python,
caption={\footnotesize \bf Implementation of \texttt{sage.DPLossValidator} used in \L\ref{list:example_pipeline}.}]
class DPLossValidator(sage.DPModelValidator):
  def validate(loss_fn, target, epsilon, confidence, B):
    if _ACCEPT_test(..., epsilon, (1-confidence)/2, B):
      return ACCEPT
    if _REJECT_test(..., epsilon, (1-confidence)/2, B):
      return REJECT
    return RETRY`{\vspace{-0.1cm}}`
  `\vspace{-0.1cm}`
  def _ACCEPT_test(test_labels, dp_test_predictions,
        loss_fn, target, epsilon, eta, B):
    n_test = dp_test_predictions.size()
    n_test_dp = n_test + laplace(2/epsilon)
    n_test_dp_min = n_test_dp - 2*log(3/(2*eta))/epsilon
    dp_test_loss = clip_by_value(loss_fn(test_labels,
      dp_test_predictions), 0, B) + laplace(2*B/epsilon)
    corrected_dp_test_loss = dp_test_loss +
      2*B*log(3/(2*eta))/epsilon
    return bernstein_upper_bound(
      corrected_dp_test_loss / n_test_dp_min,
      n_test_dp_min, eta/3, B) <= target `{\vspace{-0.1cm}}`
  `\vspace{-0.1cm}`
  def _REJECT_test(train_labels, dp_train_predictions,
        loss_fn, target, epsilon, eta, B):
    n_train = dp_train_predictions.size()
    n_train_dp = n_train + laplace(2/epsilon)
    n_train_dp_min = n_train_dp - 2*log(3/eta)/epsilon
    n_train_dp_max = n_train_dp + 2*log(3/eta)/epsilon
    dp_train_loss = clip_by_value(loss_fn(train_labels,
      dp_train_predictions), 0, B) + laplace(2*B/epsilon)
    corrected_dp_train_loss = dp_train_loss -
      2*B*log(3/(2*eta))/epsilon
    return hoeffding_lower_bound(
      corrected_dp_train_loss / n_train_dp_max,
      n_train_dp_min, eta/3, B) > target `{\vspace{-0.1cm}}`
  `\vspace{-0.1cm}`
  def bernstein_upper_bound(loss, n, eta, B):
    return loss+sqrt(2*B*loss*log(1/eta)/n)+4*log(1/eta)/n
  def hoeffding_lower_bound(loss, n, eta, B):
    return loss-B*sqrt(log(1/eta)/n)
\end{lstlisting}

\heading{General Approach.}
We have implemented SLAed validators for three classes of metrics: {\em loss metrics} (e.g. MSE for regressions), {\em accuracy metrics} (e.g. for classification), and {\em absolute errors of sum-based statistics} (e.g. mean, variance).
Appendix~\ref{appendix:sla-tests} details our implementations and proves their statistical and DP guarantees.
Here, we give the intuition and an example based on loss metrics.
All validators follow the same logic.
First, we compute a DP version of the test quantity (e.g. MSE) on a testing set.
Second, we compute the {\em worst-case impact of DP noise} on that quantity for a given confidence probability; we call this a {\em correction for DP impact}.
For example, if we add Laplace noise with parameter $\frac{1}{\epsilon}$ to the sum of squared errors on $n$ data points, assuming that the loss is in $[0,1]$ we know that with probability $(1-\eta)$ the sum is deflated by less than $-\frac{1}{\epsilon}\ln(\frac{1}{2\eta})$, because a draw from this Laplace distribution has just an $\eta$ probability to be more negative than this value.
Third, we use known statistical concentration inequalities, also made DP and corrected for worst case noise impact, to upper bound with high probability the loss on the entire distribution.

\heading{Example: Loss SLAed Validator.}
A loss function is a measure of erroneous predictions on a dataset (so lower is better).  Examples include: mean squared error for regression, log loss for classification, and minus log likelihood for Bayesian generative models.
\L\ref{list:dp_validator} shows our loss validator.
The validation function consists of two tests: {\ACCEPT} and {\REJECT}.


\underline{{\ACCEPT} Test:} Denote: the DP-trained model $\fdp$; the loss function $l$, with range $[0,B]$; the target loss $\tau_{loss}$.
Lines 11-13 compute a DP estimate of the number of samples in the test set, corrected for the impact of DP noise to be a lower bound on the true value with probability $(1-\frac{\eta}{3})$.
Lines 14-17 compute a DP estimate of the loss sum, corrected for DP impact to be an upper bound on the true value with probability $(1-\frac{\eta}{3})$.
Lines 18-20 {\ACCEPT} the model if
the upper bound is at most $\tau_{loss}$.
The bounds are based on a standard concentration inequality (specifically, Bernstein's inequality), which holds under very general conditions~\cite{Shalev-Shwartz:2014:UML:2621980}.
The Loss {\ACCEPT} Test enjoys the following guarantee (proof in Appendix~\ref{appendix:sla-tests}):



\begin{fproposition}[Loss {\ACCEPT} Test]\label{prop:loss-accept}
  With probability at least $(1-\eta)$, the {\ACCEPT} test returns true only if the expected loss of $\fdp$ is at most $\tau_{loss}$.
\end{fproposition}


\underline{{\REJECT} Test:}
The {\ACCEPT} test is already sufficient to ensure the quality of a model released by \sysname's iterative training procedure.
However, when the target is unachievable on the data distribution $\D$, these iterations waste valuable privacy resources.
The {\REJECT} test tries to detect unachievable targets so iteration can stop early.
Assuming $\fdp$ is obtained by a DP algorithm for approximately minimizing the training loss, the test detects when {\em no model} (DP or not) from the considered class $\cF$ {\em can ever hope to achieve $\tau_{loss}$} on $\D$.
The reasoning behind the test uses the fact that the minimum training loss is no more than the training loss of any $f \in \cF$; and this in particular holds for the $f^* \in \cF$ with smallest expected loss over $\D$.
With this fact, and again accounting for the DP noise and the random sampling, we prove (Appendix~\ref{appendix:sla-tests}):

\begin{fproposition}[Loss {\REJECT} Test]\label{prop:loss-reject}
With probability at least $(1-\eta)$, the {\REJECT} test returns true only if the expected loss for any $f \in \cF$ is more than $\tau_{loss}$.
\end{fproposition}



The test satisfies the preceding guarantee if invoked on the true training set loss minimizer.
Appendix~\ref{appendix:sla-tests} details and proves the precise guarantees.
In practice, we use $\fdp$ to approximate this minimizer.
If $\fdp$ is far from optimal, false rejection can happen, but this typically only happens with small sample sizes (as shown in evaluation \S\ref{sec:evaluation:slaed-model-validation}).




\iffalse
Under the assumption that $f^{np}==\hat f$, we can prove the following statistical guarantee for rejection:
\begin{fproposition}[Loss {\REJECT} Test]\label{prop:loss-reject}
  $f^{np}$ is rejected iff, with probability at least $(1-\eta)$, the best possible expected loss over the data distribution is above $\tau_{loss}$. Formally: $P(\cL_{\D}(f) \leq \tau_{loss}) \leq \eta$.
\end{fproposition}
\begin{fproof}[Proof sketch]
  $\hat f$ is the best model on the training set, so $\cL_{tr}(\hat f) \leq \cL_{tr}(f^*)$.
  Applying Hoeffding's inequality~\cite{hoeffding1963probability} gives $P(\cL_{\D}(f^*) < \cL_{tr}(f^*) -  B \sqrt{\frac{\log(3/\eta)}{n_{train}}}) \leq \frac{\eta}{3}$.
  Similarly to the proof for Proposition (\ref{prop:loss-accept}), applying a union bounds over this inequality and the DP correction gives that with probability at least $(1-\eta)$, $\cL_{\D}(f^*) \geq \cL_{tr}(f^*) -  B \sqrt{\frac{\log(3/\eta)}{n_{train}}} \geq \cL^{dp}_{tr}(\hat f) -  B \sqrt{\frac{\log(3/\eta)}{n^{min}_{tot}}} > \tau_{loss}$, concluding the proof.
\end{fproof}
\fi

\underline{DP Guarantee:}
{\ACCEPT} and {\REJECT} are individually $(\e,0)$-DP  (proofs in Appendix~\ref{appendix:sla-tests}).
They use disjoint datasets, so {\tt validate} is $(\e,0)$-DP.


\iffalse
\begin{fproposition}[DP Loss Validation]\label{prop:loss-dp}
  Running {\ACCEPT} and {\REJECT} is $(\epsilon, 0)$-DP.
\end{fproposition}
\begin{fproof}[Proof sketch]
  Each test runs on non overlapping data, so we need to show that each is DP separately.
  The only data interaction for {\ACCEPT} are to compute $n_{tot}$ and $\cL^{dp}_{te}(f)$, those are two queries with sensitivity $1$, and performing both with the Laplace noise added is $(\frac{\epsilon}{2} + \frac{\epsilon}{2}, 0)$-DP. \\
  Similarly, to show that {\REJECT} is $(\epsilon, 0)$-DP, we need to show that computing $\hat f$ and then $\cL_{tr}(f)$, has sensitivity $B$. $\hat f = \arg\min_{f\in\cF} \sum_{n_{train}} \cL_{tr}(f)$. If we add a apoint to the training set, the $\hat f$ of the previous dataset has the same loss on the points in common, and at worse how loss $B$ on the new point. The $\arg\min$ model on this new dataset can only be better, or it would not be the the $\arg\min$.  The argument when removing a point is symmetric.
  Hence the sensitivty of finding $\hat f$ and evaluating it on the training set has sensitivity $B$.
\end{fproof}
\fi


\iffalse
\heading{The Accuracy Validator} applies to classification problems, where a model predicts one out of many classes.  The target $\tau_{acc}$ is expressed in terms of accuracy, the proportion of correct
predictions.
The accuracy validator follows the same logic as the loss validator, with two small changes. First, the upper and lower bounds are reversed as losses are minimized while accuracy is maximized. Second, the result of classification predictions follows a binomial distribution, which yields tighter confidence intervals.
Note $\mathbb{1}\{\text{predicate}\}$ the indicator function with value $1$ if the predicate is true, and $0$ otherwise, and $\overline{\text{Bin}}(n_{heads}, n_{tot}, \eta)$ and $\underline{\text{Bin}}(n_{heads}, n_{tot}, \eta)$ the upper and lower bounds on the probability parameter $p$ of a binomial distribution such that $n_{heads}$ happen can happen with probability at least $\eta$ out of $n_{tot}$ independent draws (both can be conservatively approximated using a Clopper-Pearson interval).
Then, we compute $n^{te}_{true} = \sum_{n_{test}} \mathbb{1}\{f(x) = y\} + Laplace(\frac{1}{\epsilon_1})$ and $ n^{te}_{tot} =  {n_{test}} + Laplace(\frac{1}{\epsilon_2})$ (and similarly for the training set $tr$). \sysname will {\ACCEPT} when:
\[
  \underline{\text{Bin}}\Big(n_{true} - \frac{\ln(3/\eta)}{\epsilon_1}, n_{tot} + \frac{\ln(3/\eta)}{\epsilon_2}, \frac{\eta}{3}\Big) \geq \tau_{acc} .
\]
And {\REJECT} when:
\[
  \overline{\text{Bin}}\Big(n_{true} + \frac{\ln(3/\eta)}{\epsilon_1}, n_{tot} - \frac{\ln(3/\eta)}{\epsilon_2}, \frac{\eta}{3}\Big) < \tau_{acc} .
\]

Using the same reasoning, we can prove the equilalent of the three Propositions (\ref{prop:loss-accept}, \ref{prop:loss-reject}, \ref{prop:loss-dp}) for the accuracy validator.


\heading{The Sum Based Statistics Validator} applies to computations that
approximate a given sum based statistics (e.g. mean, variance). The target is
defined as the maximum size of the additive error $\tau_{err}$ for these summary
statistics on the data distribution. This error can be computed directly on the
training set, so there is no need to a test set. Second, because of the law of
large numbers, we can always reach the target precision, so there is no
rejection test.
We next show the test using Hoeffding's inequality
\cite{hoeffding1963probability} (if we expect the variance to be small,
empirical Bernstein bounds \cite{2009arXiv0907.3740M} will be better and are
directly applicable). Noting $n_{tot} = {n_{test}} + Laplace(\frac{2}{\epsilon}) -
\frac{2\log(2/\eta)}{\epsilon}$ \sysname{\ACCEPT}s if: $\frac{2\log(2/\eta)}{n_{tot}\epsilon} + B
\sqrt{\frac{\log(2/\eta)}{n_{tot}}} \leq \tau_{err}$, in which case the error of DP noise on
both the sum based summary statistic and the {\ACCEPT} test is bellow $\tau_{err}$ with probability
at least $(1-\eta)$.

\fi

